Online Multi-level Aggregation with Delays and Stochastic Arrivals

This paper presents a new research direction for online Multi-Level Aggregation (MLA) with delays. In this problem, we are given an edge-weighted rooted tree $T$, and we have to serve a sequence of requests arriving at its vertices in an online manner. Each request $r$ is characterized by two parameters: its arrival time $t(r)$ and location $l(r)$ (a vertex). Once a request $r$ arrives, we can either serve it immediately or postpone this action until any time $t > t(r)$. We can serve several pending requests at the same time, and the service cost of a service corresponds to the weight of the subtree that contains all the requests served and the root of $T$. Postponing the service of a request $r$ to time $t > t(r)$ generates an additional delay cost of $t - t(r)$. The goal is to serve all requests in an online manner such that the total cost (i.e., the total sum of service and delay costs) is minimized. The current best algorithm for this problem achieves a competitive ratio of $O(d^2)$ (Azar and Touitou, FOCS'19), where $d$ denotes the depth of the tree. Here, we consider a stochastic version of MLA where the requests follow a Poisson arrival process. We present a deterministic online algorithm which achieves a constant ratio of expectations, meaning that the ratio between the expected costs of the solution generated by our algorithm and the optimal offline solution is bounded by a constant. Our algorithm is obtained by carefully combining two strategies. In the first one, we plan periodic oblivious visits to the subset of frequent vertices, whereas in the second one, we greedily serve the pending requests in the remaining vertices. This problem is complex enough to demonstrate a very rare phenomenon that ``single-minded" or ``sample-average" strategies are not enough in stochastic optimization.

==> figures/distributed_vs_centralized.tex <==
\begin{timers}
    \def \pvar {Y}
    \def \tvar {T}
    
    \def \fstarr {2.5}
    \def \sndarr {4.25}
    \def \trdarr {6.5}
    \def \ftharr {9}
    \def \lstarr {11}
    
    \def \htime {12.5}
    \def \vtime {1.5}
    
    \def \labtimedist {0.6}
    
    % ------ distributed Poisson arrival model ------
    \coordinate (N1) at (0,0);
    
    \writelabel{$(N1)+(6.65,4.75)$}{distributed Poisson arrival model}
    
    \node (T1) at ($(N1)+(0,2*\vtime)$) {$x$};
    \node (T2) at ($(N1)+(0,\vtime)$) {$y$};
    \node (T3) at ($(N1)$) {$z$};
    \node (T4) at ($(N1)-(0,1.8)$) {};
    
    \drawarrivaltimeline{
        $(T1)+(\labtimedist,0)$ }{ \htime }{ t_x
    }{
        0/\fstarr/1/x/1, 0/\ftharr/1/x/2
    }{
        0/\fstarr/\pvar/x/1/x/1/1, \fstarr/\ftharr/\pvar/x/1/x/2/1
    }{
        \ftharr
    }{}{}{}
    \drawarrivaltimeline{
        $(T2)+(\labtimedist,0)$ }{ \htime }{ t_y
    }{
        0/\trdarr/1/y/1
    }{
        0/\trdarr/\pvar/y/1/y/1/1
    }{
        \trdarr
    }{}{}{}
    \drawarrivaltimeline{
        $(T3)+(\labtimedist,0)$ }{ \htime }{ t_z
    }{
        0/\sndarr/1/z/1, 0/\lstarr/1/z/2
    }{
        0/\sndarr/\pvar/z/1/z/1/1, \sndarr/\lstarr/\pvar/z/1/z/2/1
    }{
        \lstarr
    }{}{}{}
    
    \markrequestsbelow{
        $(T4)+(\labtimedist,0)$ }{ \htime }{ t
    }{
        1/\fstarr/1/1/, 1/\sndarr/1/2/, 1/\trdarr/1/3/, 1/\ftharr/1/4/, 1/\lstarr/1/5/
    }
    
    \coordinate (CTR) at ($(N1)+(15.35,0)$);
    \drawborder{$(CTR)+(-16.2,5.5)$}{$(CTR)+(16.2,-2.75)$}
    
    % ------ centralized Poisson arrival model ------
    \coordinate (N1) at (17,0);
    
    \writelabel{$(N1)+(6.65,4.75)$}{centralized Poisson arrival model}
    
    \node (T1) at ($(N1)+(0,2*\vtime)$) {$x$};
    \node (T2) at ($(N1)+(0,\vtime)$) {$y$};
    \node (T3) at ($(N1)$) {$z$};
    \node (T4) at ($(N1)-(0,1.8)$) {};
    
    \drawreferencelines{
        $(T3)+(\labtimedist,-0.4)$ }{ 4
    }{
        0, \fstarr, \sndarr, \trdarr, \ftharr, \lstarr
    }
    
    \drawgrayarrivaltimeline{
        $(T1)+(\labtimedist,0)$ }{ \htime }{ t_x
    }{
        0/\fstarr, 0/\ftharr
    }{
        0/\fstarr/\pvar/1, \trdarr/\ftharr/\pvar/4
    }
    \drawgrayarrivaltimeline{
        $(T2)+(\labtimedist,0)$ }{ \htime }{ t_y
    }{
        0/\trdarr/1/y/1
    }{
        \sndarr/\trdarr/\pvar/3
    }
    \drawgrayarrivaltimeline{
        $(T3)+(\labtimedist,0)$ }{ \htime }{ t_z
    }{
        0/\sndarr/1/z/1, 0/\lstarr/1/z/2
    }{
        \fstarr/\sndarr/\pvar/2, \ftharr/\lstarr/\pvar/5
    }
    
    \markrequestsandvariables{
        $(T4)+(\labtimedist,0)$ }{ \htime }{ t
    }{
        0/\fstarr/1, 0/\sndarr/2, 0/\trdarr/3, 0/\ftharr/4, 0/\lstarr/5
    }{
        0/\fstarr/\pvar/0/1,
        \fstarr/\sndarr/\pvar/0/2,
        \sndarr/\trdarr/\pvar/0/3,
        \trdarr/\ftharr/\pvar/0/4,
        \ftharr/\lstarr/\pvar/0/5
    }{
        \lstarr
    }
\end{timers}

==> figures/environments/radius.tex <==
% environment for drawing points, requests and balls
\newenvironment{radiusgraph}[0]{
    \begin{center}
    \begin{scriptsize}
    \begin{tikzpicture}[
        scale=0.25,
        every node/.style={scale=0.5},
        metric-node/.style={fill, circle, inner sep=0pt, minimum size=2.5pt},
        request-node/.style={fill, diamond, inner sep=0pt, minimum size=4pt, color=trd_main},
        empty-node/.style={circle, inner sep=0pt, minimum size=2.5pt},
        full-node/.style={fill, circle, inner sep=0pt, minimum size=2.5pt},
    ]
}{
    \end{tikzpicture}
    \end{scriptsize}
    \end{center}
}

\newcommand{\definereferencepoints}[1]{
    \coordinate (N2) at ($(#1)+(-45:1.5cm)$);
    \coordinate (N3) at ($(#1)+(-2,-2.5)$);
    \coordinate (N4) at ($(#1)+(-2,-3)$);
}

\newcommand{\drawcircles}[2]{
    \draw [draw=snd_main, fill=snd_fill, fill opacity=0.4] (N1) circle (#1cm);
    \draw [draw=fst_main, fill=fst_fill, fill opacity=0.4] (N2) circle (#2cm);
}

\newcommand{\showradiuses}[0]{
    \draw [style={->}, color=snd_main] (N1) --+(70:2cm) node[midway, right] {$\rho_x$};
    \draw [style={->}, color=fst_main] (N2) --+(160:1cm) node[midway, below] {$\rho_z$};
}

\newcommand{\connectrequests}[0]{
    \draw (N1) -- (N2);
}

\newcommand{\showfirstrequest}[0]{
    \node [request-node, label={[shift={(0.1,-0.05)}] above left:$r_1$}] (R1) at (N1) {};
}

\newcommand{\showsecondrequest}[0]{
    \node [request-node, label={[shift={(-0.1,-0.05)}] above right:$r_2$}] (R2) at (N2) {};
}

\newcommand{\drawtimeline}[1]{
    \draw [->] ($(#1)$) -- ($(#1) + (4,0)$);
    \node at ($(#1) + (4.05,-0.3)$) {\tiny{$t$}};
    
    \foreach \hl in {0,1,2,3} {
        \draw ($(#1) + (\hl,-0.06)$) -- ($(#1) + (\hl,0.06)$);
        \node at ($(#1) + (\hl,-0.35)$) {\tiny{\hl}};
    }
}

\newcommand{\showcurrenttime}[2]{
    \node [metric-node] (T) at ($(#1)+(#2,0)$) {};
}

\newcommand{\drawborder}[2]{
    \draw[rounded corners=4pt, color=gray] (#1) rectangle (#2);
}

\newcommand{\drawaxes}[7]{
    \draw[->] ($(#1) + (-0.5*#6,0)$) -- ($(#1) + (#2*#6+#6,0)$);
    \draw[->] ($(#1) + (0,-0.5*#7)$) -- ($(#1) + (0,#3*#7+#7)$);
    \node at ($(#1) + (#2*#6+#6+0.12,0)$) {\tiny{#4}};
    \node at ($(#1) + (0,#3*#7+#7+0.12)$) {\tiny{#5}};
    
    \foreach \hl in {1,2,...,#2} {
        \draw ($(#1) + (#6*\hl,-0.06)$) -- ($(#1) + (#6*\hl,0.06)$);
        \node at ($(#1) + (#6*\hl,-0.2)$) {\tiny{\hl}};
    }
    
    \foreach \vl in {1,2,...,#3} {
        \draw ($(#1) + (-0.06,#7*\vl)$) -- ($(#1) + (0.06,#7*\vl)$);
        \node at ($(#1) + (-0.45,#7*\vl)$) {\tiny{0.\vl}};
    }
}

\newcommand{\drawplotsegment}[9]{
    \draw [dashed, gray] ($(#1)+(#5,0)$) -- ($(#1)+(#5,#8)$);
    \node (P) at ($(#1)+(#5,#8+0.6)$) {$#9$};
    
    \draw [color=#2] ($(#1)+(#4,#3)$) -- ($(#1)+(#5,#3)$);
    \ifthenelse{\isodd{#6}}{\node [full-node, color=#2] (S) at ($(#1)+(#4,#3)$) {};}{}
    \ifthenelse{\isodd{#7}}{\node [empty-node, draw=#2, fill=white] (E) at ($(#1)+(#5,#3)$) {};}{}
}

\newcommand{\drawsimpleplotsegment}[7]{
    \draw [color=#2] ($(#1)+(#4,#3)$) -- ($(#1)+(#5,#3)$);
    \ifthenelse{\isodd{#6}}{\node [full-node, color=#2] (S) at ($(#1)+(#4,#3)$) {};}{}
    \ifthenelse{\isodd{#7}}{\node [empty-node, draw=#2, fill=white] (E) at ($(#1)+(#5,#3)$) {};}{}
}

==> figures/environments/small/common.tex <==
\newcommand{\writelabel}[2]{
    \node (TT) at (#1) {\normalsize{#2}};
}

\newcommand{\addtext}[1]{
    \small{#1}
}

\newcommand{\addsmalltext}[1]{
    \small{#1}
}

\newcommand{\addtinytext}[1]{
    \footnotesize{#1}
}

==> figures/environments/small/radius.tex <==
% environment for drawing points, requests and balls
\newenvironment{radiusgraph}[0]{
    \begin{center}
    \begin{scriptsize}
    \begin{tikzpicture}[
        scale=0.25,
        every node/.style={scale=0.56},
        metric-node/.style={fill, circle, inner sep=0pt, minimum size=2.5pt},
        request-node/.style={fill, diamond, inner sep=0pt, minimum size=4pt, color=trd_main},
        empty-node/.style={circle, inner sep=0pt, minimum size=2.5pt},
        full-node/.style={fill, circle, inner sep=0pt, minimum size=2.5pt},
    ]
}{
    \end{tikzpicture}
    \end{scriptsize}
    \end{center}
}

\newcommand{\definereferencepoints}[1]{
    \coordinate (N2) at ($(#1)+(-45:1.5cm)$);
    \coordinate (N3) at ($(#1)+(-2,-2.5)$);
    \coordinate (N4) at ($(#1)+(-2,-3)$);
}

\newcommand{\drawcircles}[2]{
    \draw [draw=snd_main, fill=snd_fill, fill opacity=0.4] (N1) circle (#1cm);
    \draw [draw=fst_main, fill=fst_fill, fill opacity=0.4] (N2) circle (#2cm);
}

\newcommand{\showradiuses}[0]{
    \draw [style={->}, color=snd_main] (N1) --+(70:2cm) node[midway, right] {\addtext{$\rho_x$}};
    \draw [style={->}, color=fst_main] (N2) --+(160:1cm) node[midway, below] {\addtext{$\rho_z$}};
}

\newcommand{\connectrequests}[0]{
    \draw (N1) -- (N2);
}

\newcommand{\showfirstrequest}[0]{
    \node [request-node, label={[shift={(0.1,-0.05)}] above left:\addtext{$r_1$}}] (R1) at (N1) {};
}

\newcommand{\showsecondrequest}[0]{
    \node [request-node, label={[shift={(-0.1,-0.05)}] above right:\addtext{$r_2$}}] (R2) at (N2) {};
}

\newcommand{\drawtimeline}[1]{
    \draw [->] ($(#1)$) -- ($(#1) + (4,0)$);
    \node at ($(#1) + (4.1,-0.35)$) {\addtext{$t$}};
    
    \foreach \hl in {0,1,2,3} {
        \draw ($(#1) + (\hl,-0.06)$) -- ($(#1) + (\hl,0.06)$);
        \node at ($(#1) + (\hl,-0.4)$) {\addtext{\hl}};
    }
}

\newcommand{\showcurrenttime}[2]{
    \node [metric-node] (T) at ($(#1)+(#2,0)$) {};
}

\newcommand{\drawborder}[2]{
    \draw[rounded corners=4pt, color=gray] (#1) rectangle (#2);
}

\newcommand{\drawaxes}[7]{
    \draw[->] ($(#1) + (-0.5*#6,0)$) -- ($(#1) + (#2*#6+#6,0)$);
    \draw[->] ($(#1) + (0,-0.5*#7)$) -- ($(#1) + (0,#3*#7+#7)$);
    \node at ($(#1) + (#2*#6+#6+0.12,0)$) {\addtext{#4}};
    \node at ($(#1) + (0,#3*#7+#7+0.12)$) {\addtext{#5}};
    
    \foreach \hl in {1,2,...,#2} {
        \draw ($(#1) + (#6*\hl,-0.06)$) -- ($(#1) + (#6*\hl,0.06)$);
        \node at ($(#1) + (#6*\hl,-0.2)$) {\addtext{\hl}};
    }
    
    \foreach \vl in {1,2,...,#3} {
        \draw ($(#1) + (-0.06,#7*\vl)$) -- ($(#1) + (0.06,#7*\vl)$);
        \node at ($(#1) + (-0.45,#7*\vl)$) {\addtext{0.\vl}};
    }
}

\newcommand{\drawplotsegment}[9]{
    \draw [dashed, gray] ($(#1)+(#5,0)$) -- ($(#1)+(#5,#8)$);
    \node (P) at ($(#1)+(#5,#8+0.6)$) {\addtext{$#9$}};
    
    \draw [color=#2] ($(#1)+(#4,#3)$) -- ($(#1)+(#5,#3)$);
    \ifthenelse{\isodd{#6}}{\node [full-node, color=#2] (S) at ($(#1)+(#4,#3)$) {};}{}
    \ifthenelse{\isodd{#7}}{\node [empty-node, draw=#2, fill=white] (E) at ($(#1)+(#5,#3)$) {};}{}
}

\newcommand{\drawsimpleplotsegment}[7]{
    \draw [color=#2] ($(#1)+(#4,#3)$) -- ($(#1)+(#5,#3)$);
    \ifthenelse{\isodd{#6}}{\node [full-node, color=#2] (S) at ($(#1)+(#4,#3)$) {};}{}
    \ifthenelse{\isodd{#7}}{\node [empty-node, draw=#2, fill=white] (E) at ($(#1)+(#5,#3)$) {};}{}
}

==> figures/environments/small/timers.tex <==
% environment for showing arrival times of requests
\newenvironment{timers}[0]{
    \begin{center}
    \begin{scriptsize}
    \begin{tikzpicture}[
        scale=0.25,
        every node/.style={scale=0.56},
        request-node/.style={fill, diamond, inner sep=0pt, minimum size=4pt, color=trd_main},
    ]
}{
    \end{tikzpicture}
    \end{scriptsize}
    \end{center}
}

% starting point, timeline length, timeline label, list of requests, list of waiting time intervals, endpoint of last waiting interval, color of highlighted interval, color of background for highlighted interval, list of intervals to highlight
\newcommand{\drawarrivaltimeline}[9]{
    \foreach \start/\end/\drawstart in {#9}{
        \draw [rounded corners=2pt, fill=#8, draw=none] ($(#1)+(\start,0.2)$) rectangle ($(#1)+(\end,-0.2)$);
    }

    \draw ($(#1)+(0,-0.15)$) -- ($(#1)+(0,0.15)$);
    \node (L) at ($(#1)+(#2+0.5,0)$) {\addtext{$#3$}};
    
    \foreach \mark/\arrivaltime/\labtype/\point/\number in {#4}{
        \ifthenelse{
            \isodd{\mark}
        }{
            \node [request-node] (M) at ($(#1) + (\arrivaltime,0)$) {};
        }{
            \draw [trd_main, thick] ($(#1)+(\arrivaltime,-0.12)$) -- ($(#1)+(\arrivaltime,0.12)$);
        }
        \node (R) at ($(#1) + (\arrivaltime,0.6)$) {};
    }
    
    \foreach \start/\end/\varname/\varid/\rtype/\rpoint/\rnumber/\isdone in {#5}{
        \ifthenelse{
            \isodd{\isdone}
        }{
            \draw [<->] ($(#1)+(\start,0)$) -- ($(#1)+(\end,0)$) node [midway, above] {\ifthenelse{\equal{\rtype}{0}}{\addtext{$\varname_{\varid}$}}{\ifthenelse{\equal{\rtype}{1}}{\addtext{$\varname_{\varid}^{\rnumber}$}}{\addtext{$\varname_{\varid}^{\rpoint,\rnumber}$}}}};
        }{
            \draw [<-] ($(#1)+(\start,0)$) -- ($(#1)+(\end,0)$) node [midway, above] {\ifthenelse{\equal{\rtype}{0}}{\addtext{$\varname_{\varid}$}}{\ifthenelse{\equal{\rtype}{1}}{\addtext{$\varname_{\varid}^{\rnumber}$}}{\addtext{$\varname_{\varid}^{\rpoint,\rnumber}$}}}};
            \draw ($(#1)+(\end,-0.12)$) -- ($(#1)+(\end,0.12)$);
        }
    }
    
    \draw [<->] ($(#1)+(#6,0)$) -- ($(#1)+(#2,0)$);
    
    \foreach \start/\end/\drawstart in {#9}{
        \ifthenelse{
            \isodd{\drawstart}
        }{
            \draw [<->, #7] ($(#1)+(\start,0)$) -- ($(#1)+(\end,0)$);
        }{
            \draw [->, #7] ($(#1)+(\start,0)$) -- ($(#1)+(\end,0)$);
        }
    }
    
    \node (D) at ($(#1) + (#2-0.7,0.6)$) {$\cdots$};
}

\newcommand{\markrequests}[4]{
    \draw [->] (#1) -- +(#2,0);
    \draw ($(#1)+(0,-0.15)$) -- ($(#1)+(0,0.15)$);
    \node (SV) at ($(#1)+(#2+0.5,0)$) {\addtext{$#3$}};
    
    \foreach \mark/\arrivaltime/\labtype/\point/\number in {#4}{
        \ifthenelse{
            \isodd{\mark}
        }{
            \node [request-node] (M) at ($(#1) + (\arrivaltime,0)$) {};
        }{
            \draw [trd_main, thick] ($(#1)+(\arrivaltime,-0.12)$) -- ($(#1)+(\arrivaltime,0.12)$);
        }
        \node (R) at ($(#1) + (\arrivaltime,0.6)$) {\ifthenelse{\isodd{\labtype}}{\addtext{$r_{\point}^{\number}$}}{\addtext{$r_{\number}$}}};
    }
}

\newcommand{\markrequestsbelow}[4]{
    \draw [->] (#1) -- +(#2,0);
    \draw ($(#1)+(0,-0.15)$) -- ($(#1)+(0,0.15)$);
    \node (SV) at ($(#1)+(#2+0.5,0)$) {\addtext{$#3$}};
    
    \foreach \mark/\arrivaltime/\labtype/\number/\point in {#4}{
        \ifthenelse{
            \isodd{\mark}
        }{
            \node [request-node] (M) at ($(#1) + (\arrivaltime,0)$) {};
        }{
            \draw [trd_main, thick] ($(#1)+(\arrivaltime,-0.12)$) -- ($(#1)+(\arrivaltime,0.12)$);
        }
        \node (R) at ($(#1) + (\arrivaltime,-0.6)$) {\addtext{$r_{\number}$}};
        \node (R) at ($(#1) + (\arrivaltime,0.6)$) {\addtext{$\point$}};
    }
}

\newcommand{\drawgrayarrivaltimeline}[5]{
    \draw [->, gray] (#1) -- +(#2,0);
    \draw [gray] ($(#1)+(0,-0.15)$) -- ($(#1)+(0,0.15)$);
    \node (SV) at ($(#1)+(#2+0.5,0)$) {\addtext{$#3$}};
    
    \foreach \mark/\arrivaltime in {#4}{
        \ifthenelse{
            \isodd{\mark}
        }{
            \node [request-node] (M) at ($(#1) + (\arrivaltime,0)$) {};
        }{
            \draw [trd_main, thick] ($(#1)+(\arrivaltime,-0.12)$) -- ($(#1)+(\arrivaltime,0.12)$);
        }
        \node (R) at ($(#1) + (\arrivaltime,0.6)$) {};
    }
    
    \foreach \start/\end/\varname/\varnum in {#5}{
        \draw [<->] ($(#1)+(\start,0)$) -- ($(#1)+(\end,0)$) node [midway, above] {\addtext{$\varname_{\varnum}$}};
    }
    
    \node (D) at ($(#1) + (#2-0.7,0.6)$) {\addtext{$\cdots$}};
}

\newcommand{\drawreferencelines}[3]{
    \foreach \arrival in {#3}{
        \draw [dotted, gray] ($(#1)+(\arrival,0)$) -- ($(#1)+(\arrival,#2)$);
    }
}

\newcommand{\markrequestsandvariables}[6]{
    \draw ($(#1)+(0,-0.15)$) -- ($(#1)+(0,0.15)$);
    \node (SV) at ($(#1)+(#2+0.5,0)$) {\addtext{$#3$}};
    
    \foreach \mark/\arrivaltime/\number in {#4}{
        \ifthenelse{
            \isodd{\mark}
        }{
            \node [request-node] (M) at ($(#1) + (\arrivaltime,0)$) {};
        }{
            \draw [trd_main, thick] ($(#1)+(\arrivaltime,-0.12)$) -- ($(#1)+(\arrivaltime,0.12)$);
        }
        \node (R) at ($(#1) + (\arrivaltime,-0.6)$) {\addtext{$r_{\number}$}};
    }
    
    \foreach \start/\end/\varname/\rtype/\varid/\rid in {#5}{
        \draw [<->] ($(#1)+(\start,0)$) -- ($(#1)+(\end,0)$);
        \node (L) at ($(#1)+(\start+1/2*\end-1/2*\start,0.5)$) {\ifthenelse{\isodd{\rtype}}{\addtext{$\varname_{\varid}^{\rid}$}}{\addtext{$\varname_{\varid}$}}};
    }
    
    \draw [<->] ($(#1)+(#6,0)$) -- ($(#1)+(#2,0)$);
    
    \node (D) at ($(#1) + (#2-0.7,0.6)$) {\addtext{$\cdots$}};
}


% definitions for lower bounding

% starting point, timeline length, timeline label, list of requests, list of waiting time intervals, endpoint of last waiting interval, color of highlighted interval, color of background for highlighted interval, list of intervals to highlight
\newcommand{\drawstoppedarrivaltimeline}[9]{
    \foreach \start/\end/\drawstart in {#9}{
        \draw [rounded corners=2pt, fill=#8, draw=none] ($(#1)+(\start,0.2)$) rectangle ($(#1)+(\end,-0.2)$);
    }

    \draw ($(#1)+(0,-0.15)$) -- ($(#1)+(0,0.15)$);
    
    \foreach \mark/\arrivaltime/\labtype/\point/\number in {#4}{
        \ifthenelse{
            \isodd{\mark}
        }{
            \node [request-node] (M) at ($(#1) + (\arrivaltime,0)$) {};
        }{
            \draw [trd_main, thick] ($(#1)+(\arrivaltime,-0.12)$) -- ($(#1)+(\arrivaltime,0.12)$);
        }
        \node (R) at ($(#1) + (\arrivaltime,0.6)$) {};
    }
    
    \foreach \start/\end/\varname/\varid/\rtype/\rpoint/\rnumber/\isdone in {#5}{
        \ifthenelse{
            \isodd{\isdone}
        }{
            \draw [<->] ($(#1)+(\start,0)$) -- ($(#1)+(\end,0)$) node [midway, above] {\ifthenelse{\equal{\rtype}{0}}{\addtext{$\varname_{\varid}$}}{\ifthenelse{\equal{\rtype}{1}}{\addtext{$\varname_{\varid}^{\rnumber}$}}{\addtext{$\varname_{\varid}^{\rpoint,\rnumber}$}}}};
        }{
            \draw [<-] ($(#1)+(\start,0)$) -- ($(#1)+(\end,0)$) node [midway, above] {\ifthenelse{\equal{\rtype}{0}}{\addtext{$\varname_{\varid}$}}{\ifthenelse{\equal{\rtype}{1}}{\addtext{$\varname_{\varid}^{\rnumber}$}}{\addtext{$\varname_{\varid}^{\rpoint,\rnumber}$}}}};
            \draw ($(#1)+(\end,-0.12)$) -- ($(#1)+(\end,0.12)$);
        }
    }
    
    \foreach \start/\end/\drawstart in {#9}{
        \ifthenelse{
            \isodd{\drawstart}
        }{
            \draw [<->, #7] ($(#1)+(\start,0)$) -- ($(#1)+(\end,0)$);
        }{
            \draw [->, #7] ($(#1)+(\start,0)$) -- ($(#1)+(\end,0)$);
        }
    }
}

==> figures/environments/timers.tex <==
% environment for showing arrival times of requests
\newenvironment{timers}[0]{
    \begin{center}
    \begin{scriptsize}
    \begin{tikzpicture}[
        scale=0.25,
        every node/.style={scale=0.5},
        request-node/.style={fill, diamond, inner sep=0pt, minimum size=4pt, color=trd_main},
    ]
}{
    \end{tikzpicture}
    \end{scriptsize}
    \end{center}
}

% starting point, timeline length, timeline label, list of requests, list of waiting time intervals, endpoint of last waiting interval, color of highlighted interval, color of background for highlighted interval, list of intervals to highlight
\newcommand{\drawarrivaltimeline}[9]{
    \foreach \start/\end/\drawstart in {#9}{
        \draw [rounded corners=2pt, fill=#8, draw=none] ($(#1)+(\start,0.2)$) rectangle ($(#1)+(\end,-0.2)$);
    }

    \draw ($(#1)+(0,-0.15)$) -- ($(#1)+(0,0.15)$);
    \node (L) at ($(#1)+(#2+0.5,0)$) {$#3$};
    
    \foreach \mark/\arrivaltime/\labtype/\point/\number in {#4}{
        \ifthenelse{
            \isodd{\mark}
        }{
            \node [request-node] (M) at ($(#1) + (\arrivaltime,0)$) {};
        }{
            \draw [trd_main, thick] ($(#1)+(\arrivaltime,-0.12)$) -- ($(#1)+(\arrivaltime,0.12)$);
        }
        \node (R) at ($(#1) + (\arrivaltime,0.6)$) {};
    }
    
    \foreach \start/\end/\varname/\varid/\rtype/\rpoint/\rnumber/\isdone in {#5}{
        \ifthenelse{
            \isodd{\isdone}
        }{
            \draw [stealth-stealth] ($(#1)+(\start,0)$) -- ($(#1)+(\end,0)$) node [midway, above] {\ifthenelse{\equal{\rtype}{0}}{$\varname_{\varid}$}{\ifthenelse{\equal{\rtype}{1}}{$\varname_{\varid}^{\rnumber}$}{$\varname_{\varid}^{\rpoint,\rnumber}$}}};
        }{
            \draw [stealth-] ($(#1)+(\start,0)$) -- ($(#1)+(\end,0)$) node [midway, above] {\ifthenelse{\equal{\rtype}{0}}{$\varname_{\varid}$}{\ifthenelse{\equal{\rtype}{1}}{$\varname_{\varid}^{\rnumber}$}{$\varname_{\varid}^{\rpoint,\rnumber}$}}};
            \draw ($(#1)+(\end,-0.12)$) -- ($(#1)+(\end,0.12)$);
        }
    }
    
    \draw [stealth->] ($(#1)+(#6,0)$) -- ($(#1)+(#2,0)$);
    
    \foreach \start/\end/\drawstart in {#9}{
        \ifthenelse{
            \isodd{\drawstart}
        }{
            \draw [stealth-stealth, #7] ($(#1)+(\start,0)$) -- ($(#1)+(\end,0)$);
        }{
            \draw [-stealth, #7] ($(#1)+(\start,0)$) -- ($(#1)+(\end,0)$);
        }
    }
    
    \node (D) at ($(#1) + (#2-0.7,0.6)$) {$\cdots$};
}

\newcommand{\markrequests}[4]{
    \draw [->] (#1) -- +(#2,0);
    \draw ($(#1)+(0,-0.15)$) -- ($(#1)+(0,0.15)$);
    \node (SV) at ($(#1)+(#2+0.5,0)$) {$#3$};
    
    \foreach \mark/\arrivaltime/\labtype/\point/\number in {#4}{
        \ifthenelse{
            \isodd{\mark}
        }{
            \node [request-node] (M) at ($(#1) + (\arrivaltime,0)$) {};
        }{
            \draw [trd_main, thick] ($(#1)+(\arrivaltime,-0.12)$) -- ($(#1)+(\arrivaltime,0.12)$);
        }
        \node (R) at ($(#1) + (\arrivaltime,0.6)$) {\ifthenelse{\isodd{\labtype}}{$r_{\point}^{\number}$}{$r_{\number}$}};
    }
}

\newcommand{\drawgrayarrivaltimeline}[5]{
    \draw [->, gray] (#1) -- +(#2,0);
    \draw [gray] ($(#1)+(0,-0.15)$) -- ($(#1)+(0,0.15)$);
    \node (SV) at ($(#1)+(#2+0.5,0)$) {$#3$};
    
    \foreach \mark/\arrivaltime in {#4}{
        \ifthenelse{
            \isodd{\mark}
        }{
            \node [request-node] (M) at ($(#1) + (\arrivaltime,0)$) {};
        }{
            \draw [trd_main, thick] ($(#1)+(\arrivaltime,-0.12)$) -- ($(#1)+(\arrivaltime,0.12)$);
        }
        \node (R) at ($(#1) + (\arrivaltime,0.6)$) {};
    }
    
    \foreach \start/\end/\varname/\varnum in {#5}{
        \draw [stealth-stealth] ($(#1)+(\start,0)$) -- ($(#1)+(\end,0)$) node [midway, above] {$\varname_{\varnum}$};
    }
    
    \node (D) at ($(#1) + (#2-0.7,0.6)$) {$\cdots$};
}

\newcommand{\drawreferencelines}[3]{
    \foreach \arrival in {#3}{
        \draw [dotted, gray] ($(#1)+(\arrival,0)$) -- ($(#1)+(\arrival,#2)$);
    }
}

\newcommand{\markrequestsandvariables}[6]{
    \draw ($(#1)+(0,-0.15)$) -- ($(#1)+(0,0.15)$);
    \node (SV) at ($(#1)+(#2+0.5,0)$) {$#3$};
    
    \foreach \mark/\arrivaltime/\number in {#4}{
        \ifthenelse{
            \isodd{\mark}
        }{
            \node [request-node] (M) at ($(#1) + (\arrivaltime,0)$) {};
        }{
            \draw [trd_main, thick] ($(#1)+(\arrivaltime,-0.12)$) -- ($(#1)+(\arrivaltime,0.12)$);
        }
        \node (R) at ($(#1) + (\arrivaltime,-0.6)$) {$r_{\number}$};
    }
    
    \foreach \start/\end/\varname/\rtype/\varid/\rid in {#5}{
        \draw [stealth-stealth] ($(#1)+(\start,0)$) -- ($(#1)+(\end,0)$);
        \node (L) at ($(#1)+(\start+1/2*\end-1/2*\start,0.5)$) {\ifthenelse{\isodd{\rtype}}{$\varname_{\varid}^{\rid}$}{$\varname_{\varid}$}};
    }
    
    \draw [stealth->] ($(#1)+(#6,0)$) -- ($(#1)+(#2,0)$);
    
    \node (D) at ($(#1) + (#2-0.7,0.6)$) {$\cdots$};
}


% definitions for lower bounding

% starting point, timeline length, timeline label, list of requests, list of waiting time intervals, endpoint of last waiting interval, color of highlighted interval, color of background for highlighted interval, list of intervals to highlight
\newcommand{\drawstoppedarrivaltimeline}[9]{
    \foreach \start/\end/\drawstart in {#9}{
        \draw [rounded corners=2pt, fill=#8, draw=none] ($(#1)+(\start,0.2)$) rectangle ($(#1)+(\end,-0.2)$);
    }

    \draw ($(#1)+(0,-0.15)$) -- ($(#1)+(0,0.15)$);
    
    \foreach \mark/\arrivaltime/\labtype/\point/\number in {#4}{
        \ifthenelse{
            \isodd{\mark}
        }{
            \node [request-node] (M) at ($(#1) + (\arrivaltime,0)$) {};
        }{
            \draw [trd_main, thick] ($(#1)+(\arrivaltime,-0.12)$) -- ($(#1)+(\arrivaltime,0.12)$);
        }
        \node (R) at ($(#1) + (\arrivaltime,0.6)$) {};
    }
    
    \foreach \start/\end/\varname/\varid/\rtype/\rpoint/\rnumber/\isdone in {#5}{
        \ifthenelse{
            \isodd{\isdone}
        }{
            \draw [stealth-stealth] ($(#1)+(\start,0)$) -- ($(#1)+(\end,0)$) node [midway, above] {\ifthenelse{\equal{\rtype}{0}}{$\varname_{\varid}$}{\ifthenelse{\equal{\rtype}{1}}{$\varname_{\varid}^{\rnumber}$}{$\varname_{\varid}^{\rpoint,\rnumber}$}}};
        }{
            \draw [stealth-] ($(#1)+(\start,0)$) -- ($(#1)+(\end,0)$) node [midway, above] {\ifthenelse{\equal{\rtype}{0}}{$\varname_{\varid}$}{\ifthenelse{\equal{\rtype}{1}}{$\varname_{\varid}^{\rnumber}$}{$\varname_{\varid}^{\rpoint,\rnumber}$}}};
            \draw ($(#1)+(\end,-0.12)$) -- ($(#1)+(\end,0.12)$);
        }
    }
    
    \foreach \start/\end/\drawstart in {#9}{
        \ifthenelse{
            \isodd{\drawstart}
        }{
            \draw [stealth-stealth, #7] ($(#1)+(\start,0)$) -- ($(#1)+(\end,0)$);
        }{
            \draw [-stealth, #7] ($(#1)+(\start,0)$) -- ($(#1)+(\end,0)$);
        }
    }
}

==> figures/greedy_algorithm.tex <==
\begin{radiusgraph}
    \coordinate (N1) at (0,0);
    \definereferencepoints{N1}
    \showfirstrequest
    \node [metric-node] (P2) at (N2) {};
    \drawtimeline{N3}
    \showcurrenttime{N3}{0}
    
    \coordinate (N1) at (6.6,0);
    \definereferencepoints{N1}
    \drawcircles{0.25}{0}
    \node [request-node] (R1) at (N1) {};
    \node [metric-node] (P2) at (N2) {};
    \drawtimeline{N3}
    \showcurrenttime{N3}{0.25}
    
    \coordinate (N1) at (13.2,0);
    \definereferencepoints{N1}
    \drawcircles{0.5}{0}
    \node [request-node] (R1) at (N1) {};
    \showsecondrequest
    \drawtimeline{N3}
    \showcurrenttime{N3}{0.5}
    
    \writelabel{$(N1)+(0,2.25)$}{Greedy algorithm}
    
    \coordinate (N1) at (19.8,0);
    \definereferencepoints{N1}
    \drawcircles{0.75}{0.25}
    \node [request-node] (R1) at (N1) {};
    \node [request-node] (R2) at (N2) {};
    \drawtimeline{N3}
    \showcurrenttime{N3}{0.75}
    
    \coordinate (N1) at (26.4,0);
    \definereferencepoints{N1}
    \drawcircles{1}{0.5}
    \connectrequests
    \node [request-node] (R1) at (N1) {};
    \node [request-node] (R2) at (N2) {};
    \drawtimeline{N3}
    \showcurrenttime{N3}{1}
    
    \drawborder{$(N1)+(-29,3)$}{$(N1)+(3,-3.5)$}
\end{radiusgraph}

==> figures/radius_algorithms.tex <==
\begin{radiusgraph}
    % ------ metric space and requests description ------
    \coordinate (N1) at (0,0);
    \definereferencepoints{N1}
    \drawcircles{2}{1}
    \showradiuses
    \node [metric-node, label={[shift={(0.05,-0.05)}] above left:\addtext{$x$}}] (P1) at (N1) {};
    \node [metric-node, label={[shift={(-0.05,-0.05)}] above right:\addtext{$z$}}] (P2) at (N2) {};
    
    \draw [gray] ($(N3)+(2,-0.7)$) -- +(0,-0.4);

    \node (T1) at ($(N3)+(2,-0.2)$) {\addsmalltext{$d(x,z)=1.5$}};
    \node (T2) at ($(N3)+(0.5,-0.9)$) {\addsmalltext{$\rho_x=2$}};
    \node (T3) at ($(N3)+(3.5,-0.9)$) {\addsmalltext{$\rho_z=1$}};
    
    \writelabel{$(N1)+(0,2.75)$}{metric space}
    
    \coordinate (N1) at (6.6,0);
    \definereferencepoints{N1}
    \drawcircles{2}{1}
    \showfirstrequest
    \showsecondrequest
    
    \draw [gray] ($(N3)+(2,0)$) -- +(0,-1.1);
    
    \node (T1) at ($(N3)+(0.5,-0.2)$) {\addsmalltext{$\ell(r_1)=x$}};
    \node (T2) at ($(N3)+(0.5,-0.9)$) {\addsmalltext{$t(r_1)=0$}};
    \node (T3) at ($(N3)+(3.5,-0.2)$) {\addsmalltext{$\ell(r_2)=z$}};
    \node (T4) at ($(N3)+(3.5,-0.9)$) {\addsmalltext{$t(r_2)=0.5$}};
    
    \writelabel{$(N1)+(0,2.75)$}{requests}
    
    \drawborder{$(N1)+(-9.6,3.5)$}{$(N1)+(3.1,-4.1)$}
    
    % ------ Radius algorithm ------
    \coordinate (N1) at (13.2,0);
    \definereferencepoints{N1}
    \drawcircles{2}{1}
    \showfirstrequest
    \node [metric-node] (P2) at (N2) {};
    \drawtimeline{N4}
    \showcurrenttime{N4}{0}
    
    \coordinate (N1) at (19.8,0);
    \definereferencepoints{N1}
    \drawcircles{2}{1}
    \showfirstrequest
    \showsecondrequest
    \drawtimeline{N4}
    \showcurrenttime{N4}{0.5}
    
    \writelabel{$(N1)+(0,2.75)$}{Radius algorithm}
    
    \coordinate (N1) at (26.4,0);
    \definereferencepoints{N1}
    \drawcircles{2}{1}
    \connectrequests
    \showfirstrequest
    \showsecondrequest
    \drawtimeline{N4}
    \showcurrenttime{N4}{0.5}
    
    \drawborder{$(N1)+(-16.2,3.5)$}{$(N1)+(3,-4.1)$}
\end{radiusgraph}

==> figures/radius_definition.tex <==
\begin{radiusgraph}
    \coordinate (N1) at (11.6,0);             % x
    \coordinate (N2) at ($(N1)+(150:1cm)$);   % y
    \coordinate (N3) at ($(N1)+(-80:2cm)$);   % z
    \coordinate (N4) at ($(N1)+(45:4cm)$);    % v
    \coordinate (N5) at ($(N1)+(0,-3.5)$);    % distances
    \coordinate (N6) at ($(N1)+(0,-6.1)$);    % functions
    
    \writelabel{$(N1)+(0,3.75)$}{metric space and stochastic parameters}
    
    % ------ metric space ------
    \draw [draw=snd_main, fill=snd_fill, fill opacity=0.4] (N1) circle (3cm);
    \draw [draw=fst_main, fill=fst_fill, fill opacity=0.4] (N1) circle (2cm);
    
    \draw [style={->}, color=snd_main] (N1) --+(70:3cm) node[midway, right, shift={(-0.1,-0.15)}] {\addtext{$\rho_x$}};
    \draw [style={->}, color=fst_main] (N1) --+(210:2cm) node[midway, below right, shift={(-0.1,0.05)}] {\addtext{$\rho_x'$}};
    
    \node [metric-node, label={[shift={(-0.05,0.05)}] below right:\addtext{$x$}}] (P1) at (N1) {};
    \node [metric-node, label={[shift={(-0.05,-0.1)}] above right:\addtext{$y$}}] (P2) at (N2) {};
    \node [metric-node, label={[shift={(-0.05,0.1)}] below right:\addtext{$z$}}] (P3) at (N3) {};
    \node [metric-node, label={[shift={(0,0.05)}] below:\addtext{$v$}}] (P4) at (N4) {};
    
    % ------ left parameters ------
    \coordinate (F) at ($(N1)+(-4.8,3)$);
    \textcolor{snd_main}{
        \node (T1) at ($(F)+(0,-1.5)$) {\addsmalltext{$\lambda_x = \frac{1}{6}$}};
        \node (T2) at ($(F)+(0,-2.5)$) {\addsmalltext{$\lambda_y = \frac{1}{12}$}};
        \node (T3) at ($(F)+(0,-3.5)$) {\addsmalltext{$\lambda_z = \frac{1}{12}$}};
        \node (T4) at ($(F)+(0,-4.5)$) {\addsmalltext{$\lambda_v = \frac{1}{3}$}};
    }
    
    % ------ right parameters ------
    \coordinate (F) at ($(N1)+(4.8,3)$);
    \textcolor{fst_main}{
        \node (T1) at ($(F)+(0,-1.5)$) {\addsmalltext{$\lambda_x = \frac{1}{6}$}};
        \node (T2) at ($(F)+(0,-2.5)$) {\addsmalltext{$\lambda_y = \frac{1}{5}$}};
        \node (T3) at ($(F)+(0,-3.5)$) {\addsmalltext{$\lambda_z = \frac{1}{3}$}};
        \node (T4) at ($(F)+(0,-4.5)$) {\addsmalltext{$\lambda_v = \frac{1}{2}$}};
    }
    
    % ------ distances ------
    \node (T1) at ($(N5)+(-4.5,-0.2)$) {\addsmalltext{$d(x,y)=1$}};
    \node (T2) at ($(N5)+(0,-0.2)$) {\addsmalltext{$d(x,z)=2$}};
    \node (T3) at ($(N5)+(4.5,-0.2)$) {\addsmalltext{$d(x,v)=4$}};
    
    \drawborder{$(N1)+(-6.4,4.5)$}{$(N1)+(6.4,-4.5)$}
    
    % ------ functions ------
    \node (T1) at ($(N6)+(-4,0)$) {\addtinytext{$\textcolor{snd_main}{f(u)=\dfrac{1}{\lambda\left(\bar{B}(x,u)\right)}}$}};
    \node (T2) at ($(N6)+(0,0)$) {\addtinytext{$\textcolor{trd_main}{g(u)=u}$}};
    \node (T3) at ($(N6)+(4,0)$) {\addtinytext{$\textcolor{fst_main}{f(u)=\dfrac{1}{\lambda\left(\bar{B}(x,u)\right)}}$}};
    
    \drawborder{$(N6)+(-6.5,1)$}{$(N6)+(6.5,-1)$}
    
    % ------ left graph ------
    \coordinate (G1) at (0,0);
    
    \writelabel{$(G1)+(0,3.75)$}{\textcolor{snd_main}{ball} without border points}
    
    \coordinate (Z) at ($(G1)+(-3,-5.5)$);
    \draw[->] (Z) -- ($(Z) + (6,0)$);
    \draw[->] (Z) -- ($(Z) + (0,8)$);
    
    \draw [trd_main] (Z) -- +(6,6);
    
    \node (L) at ($(Z)+(-0.6,6)$) {\addtext{$\dfrac{1}{\textcolor{snd_main}{\lambda_x}}$}};
    \node (L) at ($(Z)+(-0.6,-0.5)$) {\addtext{$0$}};
    \node (L) at ($(Z)+(6.5,0)$) {\addtext{$u$}};
    \node (L) at ($(Z)+(6.7,3/2)$) {\addtext{\textcolor{snd_main}{$f(u)$}}};
    \node (L) at ($(Z)+(6.7,6)$) {\addtext{\textcolor{trd_main}{$g(u)$}}};
    
    \draw [dotted, gray] ($(Z)+(3,0)$) -- ($(Z)+(3,7)$);
    \node (L) at ($(Z)+(3,-0.6)$) {\addtext{\textcolor{snd_main}{$\rho_x$}}};
    
    \drawplotsegment{Z}{snd_main}{6}{0}{1}{0}{1}{7}{y}
    \drawplotsegment{Z}{snd_main}{4}{1}{2}{1}{1}{7}{z}
    \drawplotsegment{Z}{snd_main}{3}{2}{4.5}{1}{1}{7}{v}
    \drawsimpleplotsegment{Z}{snd_main}{3/2}{4.5}{6}{1}{0}
    
    \draw ($(Z)+(-0.1,6)$) -- ($(Z)+(0.1,6)$);
    
    \drawborder{$(G1)+(-4.6,4.5)$}{$(G1)+(4.6,-7.1)$}
    
    % ------ right graph ------
    \coordinate (G2) at (23.2,0);
    
    \writelabel{$(G2)+(0,3.75)$}{\textcolor{fst_main}{ball} with one border point}
    
    \coordinate (Z) at ($(G2)+(-3,-5.5)$);
    \draw[->] (Z) -- ($(Z) + (6,0)$);
    \draw[->] (Z) -- ($(Z) + (0,8)$);
    
    \draw [trd_main] (Z) -- +(6,6);
    
    \node (L) at ($(Z)+(-0.6,6)$) {\addtext{$\dfrac{1}{\textcolor{fst_main}{\lambda_x}}$}};
    \node (L) at ($(Z)+(-0.6,-0.5)$) {\addtext{$0$}};
    \node (L) at ($(Z)+(6.5,0)$) {\addtext{$u$}};
    \node (L) at ($(Z)+(6.7,30/36)$) {\addtext{\textcolor{fst_main}{$f(u)$}}};
    \node (L) at ($(Z)+(6.7,6)$) {\addtext{\textcolor{trd_main}{$g(u)$}}};
    \node (L) at ($(Z)+(2,-0.6)$) {\addtext{\textcolor{fst_main}{$\rho_x'$}}};
    
    \drawplotsegment{Z}{fst_main}{6}{0}{1}{0}{1}{7}{y}
    \drawplotsegment{Z}{fst_main}{30/11}{1}{2}{1}{1}{7}{z}
    \drawplotsegment{Z}{fst_main}{30/21}{2}{4.5}{1}{1}{7}{v}
    \drawsimpleplotsegment{Z}{fst_main}{30/36}{4.5}{6}{1}{0}
    
    \drawborder{$(G2)+(-4.6,4.5)$}{$(G2)+(4.6,-7.1)$}
\end{radiusgraph}

==> figures/radius_intersection.tex <==
\begin{radiusgraph}
    \coordinate (S1) at (-0.9,0);
    \coordinate (S2) at ($(S1)+(-168:2cm)$);
    \coordinate (S3) at ($(S1)+(-25:1.8cm)$);
    
    \draw [draw=fst_main, fill=fst_fill, fill opacity=0.4] (S2) circle (1.7cm);
    \draw [draw=add_main, fill=add_fill, fill opacity=0.4] (S3) circle (1.4cm);
    \draw [draw=snd_main, fill=snd_fill, fill opacity=0.4] (S1) circle (1cm);

    \node [request-node, label={[shift={(0,-0.05)}] above:$r'$}] (R1) at (S1) {};
    \node [request-node, label={[shift={(0.1,0.05)}] below left:$r$}] (R2) at (S2) {};
    \node [request-node, label={[shift={(-0.1,0.05)}] below right:$r''$}] (R3) at (S3) {};
    
    \coordinate (S1) at (6.7,0);
    \coordinate (S2) at ($(S1)+(-160:1.2cm)$);
    
    \draw [draw=fst_main, fill=fst_fill, fill opacity=0.4] (S2) circle (1.7cm);
    \draw [draw=snd_main, fill=snd_fill, fill opacity=0.4] (S1) circle (1cm);

    \node [request-node, label={[shift={(0,-0.05)}] above:$r'$}] (R1) at (S1) {};
    \node [request-node, label={[shift={(0.1,0.05)}] below left:$r$}] (R2) at (S2) {};
    
    \writelabel{$(S1)+(-0.8,2)$}{possible scenarios for Radius}
    
    \coordinate (S1) at (12.4,0);
    \coordinate (S2) at ($(S1)+(-160:1.2cm)$);
    \coordinate (S3) at ($(S1)+(-15:2.2cm)$);
    
    \draw [draw=fst_main, fill=fst_fill, fill opacity=0.4] (S2) circle (1.7cm);
    \draw [draw=add_main, fill=add_fill, fill opacity=0.4] (S3) circle (1.4cm);
    \draw [draw=snd_main, fill=snd_fill, fill opacity=0.4] (S1) circle (1cm);

    \node [request-node, label={[shift={(0,-0.05)}] above:$r'$}] (R1) at (S1) {};
    \node [request-node, label={[shift={(0.1,0.05)}] below left:$r$}] (R2) at (S2) {};
    \node [request-node, label={[shift={(-0.1,0.05)}] below right:$r''$}] (R3) at (S3) {};
    
    \drawborder{$(-5.7,2.75)$}{$(22.8-5.7,-2.9)$}
    
    % impossible scenario
    \coordinate (S1) at (22.3,0);
    \coordinate (S2) at ($(S1)+(-160:1.2cm)$);
    \coordinate (S3) at ($(S1)+(-20:1.25cm)$);
    
    \draw [draw=fst_main, fill=fst_fill, fill opacity=0.4] (S2) circle (1.7cm);
    \draw [draw=add_main, fill=add_fill, fill opacity=0.4] (S3) circle (1.7cm);
    \draw [draw=snd_main, fill=snd_fill, fill opacity=0.4] (S1) circle (1cm);

    \node [request-node, label={[shift={(0,-0.05)}] above:$r'$}] (R1) at (S1) {};
    \node [request-node, label={[shift={(0.1,0.05)}] below left:$r$}] (R2) at (S2) {};
    \node [request-node, label={[shift={(-0.1,0.05)}] below right:$r''$}] (R3) at (S3) {};
    
    \writelabel{$(S1)+(-0.15,2)$}{impossible scenario}
    
    \drawborder{$(22.8-5.7+0.6,2.75)$}{$(22.8-5.7+0.6+9,-2.9)$}
\end{radiusgraph}

==> figures/subset_distribution.tex <==
\begin{timers}
    \def \pvar {Y}
    \def \tvar {T}
    
    \def \fstarr {3}
    \def \sndarr {5}
    \def \trdarr {8.5}
    \def \ftharr {11}
    \def \lstarr {14}
    \def \sxtarr {16.5}
    \def \svtarr {20}
    \def \etharr {22.5}
    \def \ntharr {26}
    
    \def \htime {28}
    \def \vtime {1.5}
    
    \def \labtimedist {0.6}
    
    % ------ example centralised Poisson arrival model ------
    \coordinate (N1) at (0,0);
    
    \writelabel{$(N1)+(14.6,1.75)$}{timers with resets describing centralised Poisson model}
    
    \node (T1) at (N1) {$x$};
    \node (T2) at ($(N1)+(0,-\vtime)$) {$y$};
    \node (T3) at ($(N1)+(0,-2*\vtime)$) {$z$};
    \node (T4) at ($(N1)+(0,-2*\vtime-1.8)$) {};
    
    \drawreferencelines{
        $(T3)+(\labtimedist,-0.4)$ }{ 4
    }{
        0, \fstarr, \sndarr, \trdarr, \ftharr, \lstarr, \sxtarr, \svtarr, \etharr, \ntharr
    }
    
    \drawarrivaltimeline{
        $(T1)+(\labtimedist,0)$ }{ \htime }{ t_x
    }{
        0/\fstarr/1/x/1, 0/\ftharr/1/x/2
    }{
        0/\fstarr/\tvar/x/1/x/0/1, \fstarr/\sndarr/\tvar/x/1/x/1/0, \sndarr/\trdarr/\tvar/x/1/x/2/0, \trdarr/\ftharr/\tvar/x/1/x/3/1, \ftharr/\lstarr/\tvar/x/1/x/4/0,  \lstarr/\sxtarr/\tvar/x/1/x/5/0,  \sxtarr/\svtarr/\tvar/x/1/x/6/0,  \svtarr/\etharr/\tvar/x/1/x/7/1,  \etharr/\ntharr/\tvar/x/1/x/8/0
    }{
        \ntharr}{fst_main}{fst_fill
    }{
        0/\fstarr/1, \trdarr/\ftharr/1, \svtarr/\etharr/1
    }
    \drawarrivaltimeline{
        $(T2)+(\labtimedist,0)$ }{ \htime }{ t_y
    }{
        0/\trdarr/1/y/1
    }{
        0/\fstarr/\tvar/y/1/y/0/0, \fstarr/\sndarr/\tvar/y/1/y/1/0, \sndarr/\trdarr/\tvar/y/1/y/2/1, \trdarr/\ftharr/\tvar/y/1/y/3/0, \ftharr/\lstarr/\tvar/y/1/y/4/0,  \lstarr/\sxtarr/\tvar/y/1/y/5/1,  \sxtarr/\svtarr/\tvar/y/1/y/6/0,  \svtarr/\etharr/\tvar/y/1/y/7/0,  \etharr/\ntharr/\tvar/y/1/y/8/1
    }{
        \ntharr}{fst_main}{fst_fill
    }{
        \sndarr/\trdarr/1, \lstarr/\sxtarr/1, \etharr/\ntharr/1
    }
    \drawarrivaltimeline{
        $(T3)+(\labtimedist,0)$ }{ \htime }{ t_z
    }{
        0/\sndarr/1/z/1, 0/\lstarr/1/z/2
    }{
        0/\fstarr/\tvar/z/1/z/0/0, \fstarr/\sndarr/\tvar/z/1/z/1/1, \sndarr/\trdarr/\tvar/z/1/z/2/0, \trdarr/\ftharr/\tvar/z/1/z/3/0, \ftharr/\lstarr/\tvar/z/1/z/4/1, \lstarr/\sxtarr/\tvar/z/1/z/5/0,  \sxtarr/\svtarr/\tvar/z/1/z/6/1,  \svtarr/\etharr/\tvar/z/1/z/7/0,  \etharr/\ntharr/\tvar/z/1/z/8/0
    }{
        \ntharr}{fst_main}{fst_fill
    }{
        \fstarr/\sndarr/0, \ftharr/\lstarr/0, \sxtarr/\svtarr/1
    }
    
    \markrequests{
        $(T4)+(\labtimedist,0)$ }{ \htime }{ t
    }{
        1/\fstarr/0/x/1, 1/\sndarr/0/z/2, 1/\trdarr/0/y/3, 1/\ftharr/0/x/4, 1/\lstarr/0/z/5, 1/\sxtarr/0/y/6, 1/\svtarr/0/z/7, 1/\etharr/0/x/8, 1/\ntharr/0/y/9
    }
    
    \coordinate (CTR) at ($(N1)+(14.6,0)$);
    \drawborder{$(CTR)+(-16.2,2.5)$}{$(CTR)+(16.2,-12.4)$}
    
    % ------  ------
    \coordinate (N1) at (0,-8.4);
    
    \writelabel{$(N1)+(14.6,1.75)$}{suppressed resets for point $\bar{x}$ representing $S = \{x, y\}$}
    
    \node (T1) at (N1) {$x$};
    \node (T12) at ($(N1)+(\ftharr,-1/2*\vtime)$) {};
    \node (T2) at ($(N1)+(0,-\vtime)$) {$y$};
    \node (T3) at ($(N1)+(0,-2*\vtime)$) {$z$};
    
    \drawreferencelines{
        $(T3)+(\labtimedist,-0.4)$ }{ 4
    }{
        0, \fstarr, \sndarr, \trdarr, \ftharr, \lstarr, \sxtarr, \svtarr, \etharr, \ntharr
    }
    
    \drawstoppedarrivaltimeline{
        $(T1)+(\labtimedist,0)$ }{ \htime }{ t_x
    }{
        0/\fstarr/1/x/1, 0/\ftharr/1/x/2
    }{
        0/\fstarr/\tvar/x/1/x/0/1, \fstarr/\sndarr/\tvar/x/1/x/1/0, \sndarr/\trdarr/\tvar/x/1/x/2/0, \trdarr/\ftharr/\tvar/x/1/x/3/1
    }{
        \lstarr}{fst_main}{fst_fill
    }{
        0/\fstarr/1, \trdarr/\ftharr/1
    }
    \drawstoppedarrivaltimeline{
        $(T2)+(\labtimedist,0)$ }{ \htime }{ t_y
    }{
        0/\trdarr/1/y/1
    }{
        0/\fstarr/\tvar/y/1/y/0/0, \fstarr/\sndarr/\tvar/y/1/y/1/0, \sndarr/\trdarr/\tvar/y/1/y/2/1, \trdarr/\ftharr/\tvar/y/1/y/3/0
    }{
        \lstarr}{fst_main}{fst_fill
    }{
        \sndarr/\trdarr/1
    }
    
    \drawarrivaltimeline{
        $(T12)+(\labtimedist,0)$ }{ 17 }{ t_s
    }{
        0/5.5/1/s/1, 0/11.5/1/s/2, 0/15/1/s/3
    }{
        0/5.5/\tvar/s/2/s/0/1, 5.5/11.5/\tvar/s/2/s/1/1, 11.5/15/\tvar/s/2/s/2/1
    }{
        15}{snd_main}{snd_fill
    }{
        3/5.5/0, 9/11.5/0, 11.5/15/1
    }
    \drawarrivaltimeline{
        $(T3)+(\labtimedist,0)$ }{ \htime }{ t_z
    }{
        0/\sndarr/1/z/1, 0/\lstarr/1/z/2
    }{
        0/\fstarr/\tvar/z/1/z/0/0, \fstarr/\sndarr/\tvar/z/1/z/1/1, \sndarr/\trdarr/\tvar/z/1/z/2/0, \trdarr/\ftharr/\tvar/z/1/z/3/0, \ftharr/\lstarr/\tvar/z/1/z/4/1, \lstarr/\sxtarr/\tvar/z/1/z/5/0,  \sxtarr/\svtarr/\tvar/z/1/z/6/1,  \svtarr/\etharr/\tvar/z/1/z/7/0,  \etharr/\ntharr/\tvar/z/1/z/8/0
    }{
        \ntharr}{fst_main}{fst_fill
    }{
        \fstarr/\sndarr/0, \ftharr/\lstarr/0, \sxtarr/\svtarr/1
    }
\end{timers}
